A Deep Dive into Bitcoin Mining Pools: An Empirical Analysis of Mining Shares

Miners play a key role in cryptocurrencies such as Bitcoin: they invest substantial computational resources in processing transactions and minting new currency units. It is well known that an attacker controlling more than half of the network's mining power could manipulate the state of the system at will. While the influence of large mining pools appears evenly split, the actual distribution of mining power within these pools and their economic relationships with other actors remain undisclosed. To this end, we conduct the first in-depth analysis of mining reward distribution within three of the four largest Bitcoin mining pools and examine their cross-pool economic relationships. Our results suggest that individual miners are simultaneously operating across all three pools and that in each analyzed pool a small number of actors (<= 20) receives over 50% of all BTC payouts. While the extent of an operator's control over the resources of a mining pool remains an open debate, our findings are in line with previous research, pointing out centralization tendencies in large mining pools and cryptocurrencies in general.

==> Makefile <==
####################################################
# --------------------------------------------------
# Mini Makefile for Latex papers 
# --------------------------------------------------
####################################################

# You can pass the three required variables via
# the command line without changeing the make file e.g.:
# $ FILE="template" make 

# I) File name of your LaTex source documebnt
FILE ?= ms

# II) Change this if you use latex instead of pdflatex.
# However, this also requires to update the build rules.
LATEX ?= pdflatex

# III)  
BIBTEX ?= bibtex

### rules and commands ############################

.PHONY: all
all: todoon $(FILE).pdf clean

# generate pdf and bibtex entries 
.PHONY: $(FILE).pdf
$(FILE).pdf: $(FILE).tex
	$(LATEX) $(FILE).tex
	$(BIBTEX) $(FILE)
	$(LATEX) $(FILE).tex
	$(LATEX) $(FILE).tex

# generate pdf without bibtex, in case of inline bibentries
.PHONY: inline
inline:
	$(LATEX) $(FILE).tex
	$(LATEX) $(FILE).tex
	$(LATEX) $(FILE).tex

incremental:
	latexmk -pdf -pvc $(FILE).tex

# generate pdf containing todo notes
# This temporarly changes this line in the paper:
# ```latex
# \usepackage[disable]{todonotes} % to disable/un-display all todonotes at once uncomment this
# ```
.PHONY: submission
submission: todooff $(FILE).pdf clean

.PHONY: todoon
todoon: 
	bash search_replace.sh '^\\usepackage\[disable\]{todonotes}' '\\usepackage{todonotes}'    $(FILE).tex

.PHONY: todooff
todooff:
	bash search_replace.sh '^\\usepackage{todonotes}' '\\usepackage\[disable\]{todonotes}'    $(FILE).tex

# clean als temp files
clean:
	-rm -f $(FILE).aux $(FILE).log 
	-rm -f $(FILE).bbl $(FILE).blg
	-rm -f $(FILE).nav $(FILE).out
	-rm -f $(FILE).toc $(FILE).snm
	-rm -f $(FILE).idx $(FILE).fls
	-rm -f $(FILE).ind $(FILE).ilg
	-rm -f $(FILE).fdb_latexmk $(FILE).synctex.gz

# Experimental: Generate .docx file with pandoc
#.PHONY: doc
#doc:
#	pandoc -f latex  $(FILE).tex -o $(FILE).docx


